Outlier-Resistant Estimators for Average Treatment Effect in Causal Inference

The inverse probability (IPW) and doubly robust (DR) estimators are often used to estimate the average causal effect (ATE), but are vulnerable to outliers. The IPW/DR median can be used for outlier-resistant estimation of the ATE, but the outlier resistance of the median is limited and it is not resistant enough for heavy contamination. We propose extensions of the IPW/DR estimators with density power weighting, which can eliminate the influence of outliers almost completely. The outlier resistance of the proposed estimators is evaluated through the unbiasedness of the estimating equations. Unlike the median-based methods, our estimators are resistant to outliers even under heavy contamination. Interestingly, the naive extension of the DR estimator requires bias correction to keep the double robustness even under the most tractable form of contamination. In addition, the proposed estimators are found to be highly resistant to outliers in more difficult settings where the contamination ratio depends on the covariates. The outlier resistance of our estimators from the viewpoint of the influence function is also favorable. Our theoretical results are verified via Monte Carlo simulations and real data analysis. The proposed methods were found to have more outlier resistance than the median-based methods and estimated the potential mean with a smaller error than the median-based methods.

==> table/table_MEANSD_part.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Thu Jun 03 09:46:16 2021
\begin{landscape}
  \begin{table}[ht]
  \centering
  \begin{tabular}{llccccccc}
    \hline
  &  & {\bf No contam.} & \multicolumn{3}{c}{\bf Homogeneous} \\ 
   &  &  & $\varepsilon=0.05$ & $\varepsilon=0.10$ & $\varepsilon=0.20$ \\
    \hline
 DR(T/T) & Naive & 2.999 (0.18) & 3.745 (0.60) & 4.489 (0.79) & 5.979 (1.04) \\ 
   & DP-DR ($\gamma=0.1$) & 2.998 (0.18) & 3.029 (0.30) & 3.140 (0.55) & 4.465 (1.72)  \\ 
   & DP-DR ($\gamma=0.5$) & 2.996 (0.20) & 2.997 (0.29) & 3.000 (0.33) & 3.060 (0.69)  \\ 
   & DP-DR ($\gamma=1.0$) & 2.992 (0.24) & 2.991 (0.29) & 2.992 (0.31) & 3.009 (0.52)\vspace{1mm} \\ 
   & $\varepsilon$DP-DR ($\gamma=0.1$) & 2.998 (0.18) & 3.028 (0.29) & 3.138 (0.54) & 4.464 (1.72)  \\ 
   & $\varepsilon$DP-DR ($\gamma=0.5$) & 2.996 (0.20) & 2.997 (0.26) & 2.999 (0.30) & 3.058 (0.67)  \\ 
   & $\varepsilon$DP-DR ($\gamma=1.0$) & 2.992 (0.24) & 2.991 (0.29) & 2.991 (0.30) & 3.007 (0.51)\vspace{1mm} \\ 
  DR(T/F) & Naive & 3.004 (0.24) & 3.750 (0.60) & 4.494 (0.78) & 5.984 (1.03) \\ 
   & DP-DR ($\gamma=0.1$) & 2.998 (0.24) & 3.033 (0.31) & 3.150 (0.54) & 4.490 (1.71) \\ 
   & DP-DR ($\gamma=0.5$) & 2.986 (0.25) & 2.989 (0.32) & 2.992 (0.35) & 3.059 (0.71) \\ 
   & DP-DR ($\gamma=1.0$) & 2.979 (0.28) & 2.978 (0.33) & 2.979 (0.35) & 3.001 (0.58)\vspace{1mm} \\ 
   & $\varepsilon$DP-DR ($\gamma=0.1$) & 2.998 (0.24) & 3.033 (0.31) & 3.149 (0.54) & 4.489 (1.71) \\ 
   & $\varepsilon$DP-DR ($\gamma=0.5$) & 2.986 (0.25) & 2.989 (0.32) & 2.992 (0.34) & 3.057 (0.69) \\ 
   & $\varepsilon$DP-DR ($\gamma=1.0$) & 2.979 (0.28) & 2.978 (0.33) & 2.978 (0.34) & 2.998 (0.55)\vspace{1mm} \\ 
  DR(F/T) & Naive & 2.999 (0.18) & 3.725 (0.50) & 4.451 (0.65) & 5.902 (0.86) \\ 
   & DP-DR ($\gamma=0.1$) & 2.999 (0.18) & 2.997 (0.19) & 3.051 (0.34) & 4.326 (1.57) \\ 
   & DP-DR ($\gamma=0.5$) & 3.001 (0.20) & 2.975 (0.20) & 2.950 (0.21) & 2.907 (0.35) \\ 
   & DP-DR ($\gamma=1.0$) & 3.005 (0.23) & 2.978 (0.23) & 2.953 (0.23) & 2.895 (0.25)\vspace{1mm} \\ 
   & $\varepsilon$DP-DR ($\gamma=0.1$) & 2.999 (0.18) & 3.020 (0.19) & 3.108 (0.37) & 4.541 (1.58) \\ 
   & $\varepsilon$DP-DR ($\gamma=0.5$) & 3.001 (0.20) & 2.998 (0.20) & 2.998 (0.21) & 3.020 (0.38) \\ 
   & $\varepsilon$DP-DR ($\gamma=1.0$) & 3.005 (0.23) & 3.001 (0.23) & 3.001 (0.23) & 3.003 (0.24) \\ 
   \hline
\end{tabular}
\caption{Mean and SD of 10,000 simulated estimates of $\mu^{(1)}$. The covariates $X$ were generated from Gaussian distributions, and the outcome regression was obtained by the Gaussian MLE using non-outliers. The characters "T" and "F" denote the correct and the incorrect modeling, respectively. The complete table including the IPW-type estimators and the comparative methods is Table 7 in the Appendix.}
\label{tab:exp1msd}
\end{table}
\end{landscape}

% \begin{landscape}
%   \begin{table}[ht]
%   \centering
%   \small
%   \begin{tabular}{llccccccc}
%     \hline
%   &  & {\bf No contam.} & \multicolumn{3}{c}{\bf Homogeneous} & \multicolumn{3}{c}{\bf Heterogeneous} \\ 
%   &  &  & $\varepsilon=0.05$ & $\varepsilon=0.10$ & $\varepsilon=0.20$ & $\varepsilon=0.05$ & $\varepsilon=0.10$ & $\varepsilon=0.20$ \\
%     \hline
%  DR(T/T) & Naive & 2.999 (0.18) & 3.745 (0.60) & 4.489 (0.79) & 5.979 (1.04) & 3.762 (0.64) & 4.533 (0.86) & 6.069 (1.12) \\ 
%   & DP-DR ($\gamma=0.1$) & 2.998 (0.18) & 3.029 (0.30) & 3.140 (0.55) & 4.465 (1.72) & 3.054 (0.31) & 3.207 (0.62) & 4.604 (1.78) \\ 
%   & DP-DR ($\gamma=0.5$) & 2.996 (0.20) & 2.997 (0.29) & 3.000 (0.33) & 3.060 (0.69) & 3.022 (0.27) & 3.053 (0.34) & 3.195 (0.81) \\ 
%   & DP-DR ($\gamma=1.0$) & 2.992 (0.24) & 2.991 (0.29) & 2.992 (0.31) & 3.009 (0.52) & 3.017 (0.29) & 3.047 (0.33) & 3.137 (0.66)\vspace{1mm} \\ 
%   & $\varepsilon$DP-DR ($\gamma=0.1$) & 2.998 (0.18) & 3.028 (0.29) & 3.138 (0.54) & 4.464 (1.72) & 3.054 (0.31) & 3.204 (0.60) & 4.604 (1.77) \\ 
%   & $\varepsilon$DP-DR ($\gamma=0.5$) & 2.996 (0.20) & 2.997 (0.26) & 2.999 (0.30) & 3.058 (0.67) & 3.022 (0.27) & 3.052 (0.32) & 3.190 (0.77) \\ 
%   & $\varepsilon$DP-DR ($\gamma=1.0$) & 2.992 (0.24) & 2.991 (0.29) & 2.991 (0.30) & 3.007 (0.51) & 3.017 (0.29) & 3.047 (0.33) & 3.134 (0.63)\vspace{1mm} \\ 
%   DR(T/F) & Naive & 3.004 (0.24) & 3.750 (0.60) & 4.494 (0.78) & 5.984 (1.03) & 3.767 (0.64) & 4.537 (0.85) & 6.073 (1.09) \\ 
%   & DP-DR ($\gamma=0.1$) & 2.998 (0.24) & 3.033 (0.31) & 3.150 (0.54) & 4.490 (1.71) & 3.060 (0.32) & 3.218 (0.61) & 4.624 (1.76) \\ 
%   & DP-DR ($\gamma=0.5$) & 2.986 (0.25) & 2.989 (0.32) & 2.992 (0.35) & 3.059 (0.71) & 3.014 (0.32) & 3.044 (0.36) & 3.196 (0.82) \\ 
%   & DP-DR ($\gamma=1.0$) & 2.979 (0.28) & 2.978 (0.33) & 2.979 (0.35) & 3.001 (0.58) & 3.004 (0.33) & 3.035 (0.37) & 3.133 (0.70)\vspace{1mm} \\ 
%   & $\varepsilon$DP-DR ($\gamma=0.1$) & 2.998 (0.24) & 3.033 (0.31) & 3.149 (0.54) & 4.489 (1.71) & 3.059 (0.32) & 3.218 (0.60) & 4.623 (1.75) \\ 
%   & $\varepsilon$DP-DR ($\gamma=0.5$) & 2.986 (0.25) & 2.989 (0.32) & 2.992 (0.34) & 3.057 (0.69) & 3.013 (0.31) & 3.044 (0.35) & 3.192 (0.79) \\ 
%   & $\varepsilon$DP-DR ($\gamma=1.0$) & 2.979 (0.28) & 2.978 (0.33) & 2.978 (0.34) & 2.998 (0.55) & 3.004 (0.33) & 3.035 (0.37) & 3.132 (0.70)\vspace{1mm} \\ 
%   DR(F/T) & Naive & 2.999 (0.18) & 3.725 (0.50) & 4.451 (0.65) & 5.902 (0.86) & 3.667 (0.49) & 4.341 (0.65) & 5.685 (0.84) \\ 
%   & DP-DR ($\gamma=0.1$) & 2.999 (0.18) & 2.997 (0.19) & 3.051 (0.34) & 4.326 (1.57) & 3.018 (0.19) & 3.077 (0.29) & 4.000 (1.35) \\ 
%   & DP-DR ($\gamma=0.5$) & 3.001 (0.20) & 2.975 (0.20) & 2.950 (0.21) & 2.907 (0.35) & 3.000 (0.20) & 3.000 (0.21) & 3.008 (0.28) \\ 
%   & DP-DR ($\gamma=1.0$) & 3.005 (0.23) & 2.978 (0.23) & 2.953 (0.23) & 2.895 (0.25) & 3.004 (0.23) & 3.006 (0.23) & 3.008 (0.24)\vspace{1mm} \\ 
%   & $\varepsilon$DP-DR ($\gamma=0.1$) & 2.999 (0.18) & 3.020 (0.19) & 3.108 (0.37) & 4.541 (1.58) & 3.040 (0.19) & 3.131 (0.31) & 4.209 (1.39) \\ 
%   & $\varepsilon$DP-DR ($\gamma=0.5$) & 3.001 (0.20) & 2.998 (0.20) & 2.998 (0.21) & 3.020 (0.38) & 3.022 (0.20) & 3.048 (0.21) & 3.117 (0.30) \\ 
%   & $\varepsilon$DP-DR ($\gamma=1.0$) & 3.005 (0.23) & 3.001 (0.23) & 3.001 (0.23) & 3.003 (0.24) & 3.027 (0.23) & 3.054 (0.23) & 3.116 (0.23) \\ 
%   \hline
% \end{tabular}
% \caption{Mean and SD of 10,000 simulated estimates of $\mu^{(1)}$. The covariates $X$ were generated from Gaussian distributions, and the outcome regression was obtained by the Gaussian MLE using non-outliers. The characters "T" and "F" denote the correct and the incorrect modeling, respectively. The complete table including the IPW-type estimators and the comparative methods is available in the Appendix.}
% \label{tab:exp1msd}
% \end{table}
% \end{landscape}



